Understanding and Robustifying Differentiable Architecture Search

Differentiable Architecture Search (DARTS) has attracted a lot of attention due to its simplicity and small search costs achieved by a continuous relaxation and an approximation of the resulting bi-level optimization problem. However, DARTS does not work robustly for new problems: we identify a wide range of search spaces for which DARTS yields degenerate architectures with very poor test performance. We study this failure mode and show that, while DARTS successfully minimizes validation loss, the found solutions generalize poorly when they coincide with high validation loss curvature in the architecture space. We show that by adding one of various types of regularization we can robustify DARTS to find solutions with less curvature and better generalization properties. Based on these observations, we propose several simple variations of DARTS that perform substantially more robustly in practice. Our observations are robust across five search spaces on three image classification tasks and also hold for the very different domains of disparity estimation (a dense regression task) and language modelling.

==> deprecated.tex <==
\begin{figure}
{
     \begin{minipage}{.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{figures/section_6/argmax_test.pdf}
     \captionof{figure}{Drop in accuracy after discretizing the search model for different spaces, datasets and drop path regularization strengths.. Example of some of the settings from Section \ref{sec:regularizing_inner}.}
     \label{fig:dp_drop}
    \end{minipage}
    ~~
    \begin{minipage}{.48\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/section_4/corr_s1_c10_mean.pdf}
      \captionof{figure}{Correlation between dominant eigenvalue  of $\nabla^2_{\alpha}\mathcal{L}_{valid}$ and test error of corresponding architectures.}
      %from running standard DARTS and our regularized versions.}
      \label{fig:val_eig_correlation}
    \end{minipage}
}
\end{figure}

==> section_5.tex <==
\section{Discussion and further analysis}
\label{discussion}
\tce{we should look for a more meaningful title. we should also describe how this relates to the previous sections as the red line is not so clear right now}
In this section we discuss one potential hypothesis that may explain why DARTS fails in several scenarios as shown in this paper. Afterwards we provide empirical justification on why the curvature of the validation objective is a good indicator for the generalization performance of the architectures found by DARTS.

As it is well known in the settings of large vs. small batch training~\citep{yao18,Keskar16,Hochreiter97},\tce{todo} one potential hypothesis explaining the relationship between the sharpness of minima and generalization properties of a neural network, is based on the fact that the training function is much more sensitive at a sharp minimizer, e.g. to the variations in the input data. This may lead to relatively large accuracy drop even from small discrepancies between training and test data.
Analogously, we conjectured that this also holds for $\alpha$ rather than $w$ and therefore we investigated the relation between large eigenvalues (w.r.t. $\alpha$) - as a proxy for sharp minima - and generalization performance. Similarly, sharp minima would also be much more sensitive to variations in the architecture, which is relevant since DARTS discretizes (by taking the \emph{argmax} over operations in each edge) the optimal $\alpha^*$ after search, resulting in $\alpha^d$ somewhere in the neighbourhood of $\alpha^*$. In the case of a sharp minimum $\alpha^*$, $\alpha^d$ might already have a significantly larger objective function value, while in the case of a flat minimum, $\alpha^d$ is expected to have an objective value similar to $\alpha^*$.

\begin{wrapfigure}[26]{r}{0.4\textwidth}
\vskip -0.24in
  \centering
  \includegraphics[width=.4\textwidth]{figures/section_6/scatter_argmax.pdf}\\
  \includegraphics[width=.4\textwidth]{figures/section_6/argmax_test.pdf}
  \caption{Drop in accuracy after discretizing the search model. (\textit{Top}) Correlation with the landscape curvature. (\textit{Bottom}) Example of some of the settings from Section \ref{sec:regularizing_inner}.}
  \label{fig:argmax_evaluation}
\end{wrapfigure}

To make this more crisp, we conducted the following experiment: after the DARTS search has finished, we discretize the architecture and evaluate it with the search model's weights, rather than retraining, and compare the performance to the one-shot model's performance. Figure \ref{fig:argmax_evaluation} (\textit{bottom}) shows the drop in performance due to this discretization step for some of the settings: this drop is much larger when there is little regularization (drop prob = 0), resulting in large eigenvalues (see Figures \ref{fig:eigenspectrum_dp} and \ref{fig:eigenspectrum_wd} Appendix), corresponding to a sharp minimum. Figure \ref{fig:argmax_evaluation} (\textit{top}) shows the relationship between the dominant eigenvalues at the end of search and the drop in accuracy when doing the discretization step as described above.
\tce{I'm not sure if we want to keep the next paragraph. It's not too related to the previous one.}
Why does DARTS get attracted to these bad regions in the architecture space? This might arise potentially from some premature convergence in the weights' space, supposing that the landscape of the training loss $\mathcal{L}_{train}$ does not change significantly after each $\alpha$ update. In a non-convex landscape, this minimizer $w^{(1)}$ of $\mathcal{L}_{train}$ might not necessarily be the one that also minimizes $\mathcal{L}_{valid}$ (see \citet{franceschi18a}), i.e. there might exist another $w^{(2)} \in \argmin_{w} \mathcal{L}_{train}(\alpha, w)$ such that $\mathcal{L}_{valid}(\alpha, w^{(2)}) < \mathcal{L}_{valid}(\alpha, w^{(1)})$. More concretely, the parameterless operations such as \textit{skip connections} might get higher weight especially in the beginning of search due to the easiness of gradients to flow through these paths during training. Regularizing the inner objective by adding a convex term or perturbing the inputs will eventually redirect also the gradients flowing backwards, and consecutively also the attention DARTS focuses on different architectural operations.



==> section_6.tex <==
\section{Practical Robustification of DARTS}
\label{sec:practical}
\tce{IMO, this whole section (except DARTS-ADA) doesnt contribute a lot but it costs much space. I'd put DARTS-ADA in Section 5 and extend TAble 1.}
While we demonstrated in Section \ref{sec:regularizing_inner} that additional regularization serves to robustify DARTS, the regularization by L2 penalty and data augmentation introduces additional hyperparameters. While one could of course run an extensive optimization of these for each dataset at a time, this is not useful for practical applications since the runtime for this routine would have to be counted as part of the runtime of the resulting method~\citep{best_practices}. Rather, in this section, we propose practical robustification methods that come with minimal computational overhead.

\subsection{DARTS with adaptive regularization}
\label{sec: DARTS_ADA}
\tce{maybe make this 5.3?}
Based on the insights from the aforementioned analysis and empirical results, one may think of a way to adapt DARTS' hyperparameters ($L_2$ regularization or max. drop path probability value)  in an automated way, in order to keep the architectural weights in areas of the validation loss objective with smaller curvature. The simplest off-the-shelf procedure towards this desiderata would be to increase the regularization strength whenever the dominant eigenvalue starts increasing rapidly.

Algorithm \ref{alg: DARTS_ADA} (DARTS-ADA, see the Appendix) shows such a procedure. We use the same criterion ($\texttt{stop\_criter}$) used in the DARTS-ES (Section \ref{reg:early_stop}), roll back DARTS to the architectural and search model parameters at that point ($\texttt{stop\_epoch}$) whenever this criterion is met, and continue the search with a larger regularization value $R$ for the remaining epochs (larger by a factor of $\eta$). This procedure is repeated whenever the criterion is met, unless the regularization value exceeds some maximum predefined value $R_{max}$. 

\subsection{A Simple Robustification of DARTS}
\label{sec:RobustDARTS}

In order to hedge against brittle optimization runs, the original DARTS paper~\citep{liu-iclr18} already suggested to run the search phase of DARTS four times, resulting in four architectures, and to return the best of these four architectures w.r.t.\ validation performance when retrained  from scratch for a limited number of epochs. 
Then the returned architecture is retrained from scratch as usual, for 600 epochs using the evaluation settings (see Appendix \ref{sec: arch_eval}).
We propose to use the same procedure, with the only difference that the four runs of the search phase use different amounts of regularization. The resulting RobustDARTS (R-DARTS) method is conceptually very simple, trivial to implement, and likely to work well if any of the tried regularization strengths works well.

\subsection{Empirical Evaluation}
\label{sec:empirical}

\begin{table}[t]
\begin{small}
\centering
\vskip -0.47in
\caption{Empirical evaluation of practical robustified versions of DARTS. Each entry is the test error after retraining the selected architecture as described in Section \ref{sec:RobustDARTS}.}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Setting}} & \textbf{RS-ws} & \textbf{DARTS} & \textbf{R-DARTS(DP)} & \textbf{R-DARTS(L2)} & \textbf{DARTS-ES} & \textbf{DARTS-ADA} \\ \hline\hline
\multirow{4}{*}{C10}       & S1 & 3.23  &  3.84  & 3.11 & \underline{\textbf{2.78}}   &  \textbf{3.01}  &  3.10      \\ \cline{2-8} 
                           & S2 & 3.66  &  4.85  &  3.48  &  \textbf{3.31}     &  \underline{\textbf{3.26}}  &  3.35      \\ \cline{2-8} 
                           & S3 & 2.95  &  3.34  &  2.93  &  \underline{\textbf{2.51}}   &  2.74  &  \textbf{2.59}      \\ \cline{2-8} 
                           & S4 & 8.07  &  7.20  &  \textbf{3.58}  &  \underline{\textbf{3.56}}    &  3.71  &  4.84      \\ \hline\hline
\multirow{4}{*}{C100}      & S1 & \underline{\textbf{23.30}} &  29.46 &  25.93  &  24.25  &  28.37 &  \textbf{24.03}     \\ \cline{2-8} 
                           & S2 & \underline{\textbf{21.21}} &  26.05 &  22.30  &  \textbf{22.24}  &  23.25 &  23.52     \\ \cline{2-8} 
                           & S3 & 23.75 &  28.90 &  \underline{\textbf{22.36}}  &  23.99  &  23.73 &  \textbf{23.37}     \\ \cline{2-8} 
                           & S4 & 28.19 &  22.85 &  22.18  &  \textbf{21.94}  &  \underline{\textbf{21.26}} &  23.20     \\ \hline\hline
\multirow{4}{*}{SVHN}      & S1 & 2.59  &  4.58 &  \textbf{2.55}  &  4.79   &  2.72  &  \underline{\textbf{2.53}}      \\ \cline{2-8} 
                           & S2 & 2.72  &  3.53  & \textbf{2.52}  &  \underline{\textbf{2.51}}   &  2.60  &  2.54      \\ \cline{2-8} 
                           & S3 & 2.87  &  3.41  & \textbf{2.49}  &  \underline{\textbf{2.48}}   &  2.50  &  2.50      \\ \cline{2-8} 
                           & S4 & 3.46  &  3.05  & 2.61  &  \textbf{2.50}   &  2.51  &  \underline{\textbf{2.46}}      \\ \hline
\end{tabular}
\label{tab:robust_darts}
\end{small}
\end{table}

Table \ref{tab:robust_darts} evaluates the performance of our practical robustifications of DARTS, DARTS-ADA and R-DARTS (based on either L2 or ScheduledDropPath regularization), by comparing them to the original DARTS, DARTS-ES and Random Search with weight sharing (RS-ws). 
For each of these methods, as proposed in the DARTS paper~\citep{liu-iclr18}, we ran the search four independent times with different random seeds and selected the architecture used for the final evaluation based on a validation run as described above.
As the table shows, in accordance with \citet{Li19}, RS-ws often outperforms the original DARTS; however, with our robustifications, DARTS typically performs substantially better than RS-ws.
The improvements of DARTS-ADA are consistent across all settings compared to the default DARTS, indicating that a gradual increase of regularization during search prevents ending up in the bad regions of the architectural space.
%
Finally, RobustDARTS yielded the best performance and since it is also easier to implement than DARTS-ES and DARTS-ADA, it is the method that we recommend to be used in practice.

